RIVER: A Real-Time Interaction Benchmark for Video LLMs

The rapid advancement of multimodal large language models has demonstrated impressive capabilities, yet nearly all operate in an offline paradigm, hindering real-time interactivity. Addressing this gap, we introduce the Real-tIme Video intERaction Bench (RIVER Bench), designed for evaluating online video comprehension. RIVER Bench introduces a novel framework comprising Retrospective Memory, Live-Perception, and Proactive Anticipation tasks, closely mimicking interactive dialogues rather than responding to entire videos at once. We conducted detailed annotations using videos from diverse sources and varying lengths, and precisely defined the real-time interactive format. Evaluations across various model categories reveal that while offline models perform well in single question-answering tasks, they struggle with real-time processing. Addressing the limitations of existing models in online video interaction, especially their deficiencies in long-term memory and future perception, we proposed a general improvement method that enables models to interact with users more flexibly in real time. We believe this work will significantly advance the development of real-time interactive video understanding models and inspire future research in this emerging field. Datasets and code are publicly available at https://github.com/OpenGVLab/RIVER.

==> sec/4_model.tex <==
\section{Model}
\label{sec:model}
% 4.1基础模型
% 我们使用videochat2-next作为我们的基础模型。我们在videollm-Online的基础上进行改进，使用SigLip-so-400m作为视觉编码器提取frame特征。经过一层mlp，frame特征被映射到LLM的language embedding空间。随后，visual-text interleaved数据被送入LLM，以自回归方式进行理解和输出，其中Llama3-8B作为语言模型LLM。
% 区别于传统的视频理解模型，我们的在线模型可以在某些问题提出后产生停顿并选择合适的时机再作出响应。特殊的token End-of-Sequence (EOS)被引入训练数据，以达到停顿的效果。具体的，语言建模可以表示为如下形式
% max P ([Txt t i+1]|[Ctx <t ], [Frame t ], [Txt t ≤i])
% 其中，Txt代表文本，Ctx代表此前对话的所有内容，i代表文本的第i个token。当EOS的next-token概率达到一定阈值时，模型将不进行输出。
% 经过训练，原来的离线视频理解模型获得了很强的在线视频理解能力。我们改变了它作为普通离线模型的对话形式，在原有视频理解能力基础上，增强了在线交互的能力。训练数据生成自ego4d的training set，制作流程和bench一样，数量大约为30k，足够赋予模型新的能力。
% 4.2离线改在线
% 针对纯离线模型，我们采用滑窗和记忆模块结合的方法提升其在线理解和交互的能力。
% 相比于离线模型的原始理解方式，将整个视频流输入并回答问题，滑窗的方式允许模型与user进行多次交互，提升了模型实时响应的能力。另外通过借鉴videoAgent中的prompt，模型在每个窗口进行思考和判断，像agent一样具有了自主判断是否响应的能力。这种实时响应是实际应用中最迫切需要的，同时也是离线模型非常欠缺的，然而，在每个滑窗进行提问将会导致大量的时间与计算消耗。
% 在记忆模块部分，我们采用moviechat中提出的long-short term memory机制来提升模型的回忆能力。短期记忆由模型对当前窗口内的视觉信息进行编码得到，短期记忆部分使用模型的原始配置，以最大程度地保留模型自身的视频理解能力。长期记忆部分由于要保留很多过去帧的信息，占用存储较多，所以相邻的patch token将被合并为一个，以减少总token数。当新的frames feature输入后，选择性地保留包含更多有效信息的feature。最终，将这长短期记忆信息合并、共同输入projector和LLM，使得模型可以感知更长时间跨度的视觉信息。
\subsection{online model}

We employ VideoChat2-Next as our base model. Building upon VideoLLM-Online, we utilize SigLip-SO-400M as the visual encoder to extract frame features. These frame features are then mapped to the language embedding space of the large language model (LLM) through a multi-layer perceptron (MLP). Subsequently, the visual-text interleaved data is fed into the LLM, which processes and generates outputs in an autoregressive manner. Here, Llama3-8B serves as the LLM.

Unlike traditional video understanding models, our online model can pause after certain questions are posed and choose an appropriate moment to respond. A special token, End-of-Sequence (EOS), is introduced into the training data to achieve this pausing effect. Specifically, the language modeling can be expressed as:

$$
\max P \left( [\text{Txt}_{t}^{i+1}] \,|\, [\text{Ctx}_{<t}], [\text{Frame}_t], [\text{Txt}_t^{\leq i}] \right),
$$
where Txt represents the text, Ctx denotes all previous dialogue content, and \( i \) represents the \( i \)-th token of the text. When the next-token probability of EOS reaches a certain threshold, the model ceases to generate further output.

Through training, the original offline video understanding model acquires robust online video understanding capabilities. We modify its dialogue format from that of a conventional offline model, enhancing its interactive abilities while retaining its foundational video comprehension skills. The training data, generated from the Ego4D training set, follows a similar construction process to the benchmark and comprises approximately 30,000 instances, which is sufficient to endow the model with new capabilities.

\subsection{Adapting Offline Models for Online Use}

For purely offline models, we enhance their online understanding and interaction capabilities by combining a sliding window approach with a memory module.

Compared to the original offline model's approach of processing the entire video stream before answering questions, the sliding window method allows the model to interact with the user multiple times, significantly improving its real-time responsiveness. Additionally, by incorporating prompts inspired by VideoAgent, the model can deliberate and make decisions within each window, akin to an agent, autonomously determining whether to respond. This real-time responsiveness is critically needed in practical applications and is a significant limitation of traditional offline models. However, querying within each sliding window can lead to substantial time and computational overhead.

For the memory module, we adopt the long-short term memory mechanism proposed in MovieChat to enhance the model's recall capabilities. Short-term memory is derived from the model's encoding of visual information within the current window, utilizing the model's original configuration to preserve its inherent video understanding capabilities to the greatest extent. Long-term memory, which retains information from many past frames, requires more storage. To reduce the total number of tokens, adjacent patch tokens are merged into one. When new frame features are input, features containing more relevant information are selectively retained. Finally, the combined long- and short-term memory information is fed into the projector and LLM, enabling the model to perceive visual information over longer time spans. 

This adaptation not only improves the model's ability to handle real-time interactions but also ensures efficient utilization of computational resources, making it more suitable for practical online video understanding applications.







